Challenges in Multi-centric Generalization: Phase and Step Recognition in Roux-en-Y Gastric Bypass Surgery

Most studies on surgical activity recognition utilizing Artificial intelligence (AI) have focused mainly on recognizing one type of activity from small and mono-centric surgical video datasets. It remains speculative whether those models would generalize to other centers. In this work, we introduce a large multi-centric multi-activity dataset consisting of 140 videos (MultiBypass140) of laparoscopic Roux-en-Y gastric bypass (LRYGB) surgeries performed at two medical centers: the University Hospital of Strasbourg (StrasBypass70) and Inselspital, Bern University Hospital (BernBypass70). The dataset has been fully annotated with phases and steps. Furthermore, we assess the generalizability and benchmark different deep learning models in 7 experimental studies: 1) Training and evaluation on BernBypass70; 2) Training and evaluation on StrasBypass70; 3) Training and evaluation on the MultiBypass140; 4) Training on BernBypass70, evaluation on StrasBypass70; 5) Training on StrasBypass70, evaluation on BernBypass70; Training on MultiBypass140, evaluation 6) on BernBypass70 and 7) on StrasBypass70. The model's performance is markedly influenced by the training data. The worst results were obtained in experiments 4) and 5) confirming the limited generalization capabilities of models trained on mono-centric data. The use of multi-centric training data, experiments 6) and 7), improves the generalization capabilities of the models, bringing them beyond the level of independent mono-centric training and validation (experiments 1) and 2)). MultiBypass140 shows considerable variation in surgical technique and workflow of LRYGB procedures between centers. Therefore, generalization experiments demonstrate a remarkable difference in model performance. These results highlight the importance of multi-centric datasets for AI model generalization to account for variance in surgical technique and workflows.

==> media_temp_arxiv.tex <==
%%
%% This is file `medima.sty',
%% generated with the docstrip utility.
%%
%% Copyright 2018 Elsevier Ltd
%% 
%% This file is part of the 'Elsarticle Bundle'.
%% -------------------------------------------
%% 
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%% 
%%
%% $Id: medima.sty 141 2018-09-06 09:48:47Z rishi $
%% $URL: http://lenova.river-valley.com/svn/elsarticle/trunk/medima.sty $
%%
 \def\RCSfile{medima}%
 \def\RCSversion{0.1}%
 \def\RCSdate{2018/09/01}%
 \def\@shortjnl{\relax}
 \def\@journal{Medical Image Analysis}
 \def\@company{Elsevier B. V.}
 \def\@issn{1361-8415}
 \def\@shortjid{medima}
\NeedsTeXFormat{LaTeX2e}[1995/12/01]

\@ifclassloaded{elsarticle}
{\typeout{elsarticle.cls is loaded...}}
{\errmessage{This package will work only with 
  elsarticle.cls. So please load elsarticle.cls 
  and try.}}
  
\@ifpackageloaded{hyperref}{}
   {\def\href#1#2{#2}}  

\@ifundefined{@makefntext}{\let\@makefntext\relax}{}
  
\AtBeginDocument{\@twosidetrue\@mparswitchtrue}

\def\@verso{}
\gdef\verso#1{\gdef\@verso{#1}}

\gdef\baselinestretch{1}%
\gdef\belowabstractskip{10pt}%

 \RequirePackage{geometry}
 \geometry{twoside,
  paperwidth=210mm,
  paperheight=280mm,
  textheight=635.35pt,
  textwidth=467.75pt,
  inner=32pt,
  outer=43pt,
  top=65pt,
  bottom=40pt,
  headheight=12pt,
  headsep=12pt,
  footskip=16pt,
  footnotesep=28pt plus 2pt minus 6pt,
  columnsep=18pt
 }
 \global\let\bibfont=\footnotesize
 \global\bibsep=0pt
 \input{fleqn.clo}
%\ifpreprint
%\else
%   \global\@twocolumntrue
%\fi

\long\def\elsputbox(#1)(#2)[#3]#4{%
       \unitlength=1mm%
       \fboxsep=-\fboxrule
       \fboxrule0pt%
       \fboxsep0pt%
       \ifvmode\leavevmode\fi\smash{\put(#1)%
       {\makebox(#2)[#3]{\fbox{#4}}}}}
       
\long\def\elsptputbox(#1)(#2)[#3]#4{%
       \unitlength=1pt%
       \fboxsep=-\fboxrule
       \fboxrule0pt%
       \fboxsep0pt%
       \ifvmode\leavevmode\fi\smash{\put(#1)%
       {\makebox(#2)[#3]{\fbox{#4}}}}}

\usepackage{multirow}
\usepackage{color}

\definecolor{gray10}{gray}{.9}

\AtBeginDocument{
\def\elsarticletitlealign{flushleft}
}

%%
\def\snm#1{\textcolor{black}{#1}}

% \def\tnotemark[#1]{\@for\mytmark:=#1\do{%
%       \@ifundefined{X@\mytmark}%
%           {\expandafter\def\csname X@\mytmark\endcsname{0}}%
%           {}%
%       \expandafter\ifcase\csname X@\mytmark\endcsname\or$^{\star}$\or
%       $^{,\star\star}$\fi
%     }%
% }

\def\elstitleheaderwidth{\textwidth}%165mm
% \def\titleboxawidth{159.5mm}
% \def\elsjnllogowidth{20mm}
% \def\titleblocksep{4mm}%
% \def\titlegrayboxwidth{132.5mm}
% \def\titlegrayboxheight{20.75mm}
% \def\elsjnllogoheight{25.24mm}
% \def\elstitleboxcolor{gray10}
% \def\ScienceDirect{\href{http://www.sciencedirect.com}{ScienceDirect}}
% \if@twocolumn%
%   \def\abovestmtitleheaderskip{-16pt}%
% \else%
%   \def\abovestmtitleheaderskip{-28pt}%
% \fi%
% \def\crossmarkskip{25mm}
% \def\jnllogo{medima-logo}
% \def\elslogo{elsevier-logo}
% \def\jnlurl#1{\gdef\@jnlurl{#1}}
% \gdef\@jnlurl{www.elsevier.com/locate/media}

% \def\elstitleheadboxa#1#2#3{%
%     \minipage[b][][t]{#1}%
%      \hrule width #1 height 0.3pt%
%      \vspace*{6pt}%
%       {\raisebox{-3pt}{\includegraphics%
%           {\elslogo}\hspace*{\titleblocksep}}}%
%      \colorbox{\elstitleboxcolor}{%     
%       \parbox[b][#2]{#3}{\elstitlejnldetails}}%
%   \endminipage%
}

\def\elstitlejnldetails{%
    \minipage[b][23mm][b]{\titlegrayboxwidth}%
       \centering%
       \parbox[b]{\titlegrayboxwidth}{%       
       \centering\sffamily%
       \fontsize{8.5pt}{9.6pt}\fontseries{m}\selectfont%       
       Contents lists available at \ScienceDirect}\\[15pt]%
       {\fontsize{15pt}{18pt}\selectfont%
        % \@journal%
       }\\[15pt]%
       \parbox[b]{\titlegrayboxwidth}%
       {\centering\sffamily\fontsize{8.5pt}{9.6pt}\fontseries{m}\selectfont%       
       journal homepage:~%
       \href{http://\@jnlurl}{\@jnlurl}%
       \vspace*{0pt}%
       }%
      \endminipage}

\def\elsjnllogoboxb#1#2{%
  \minipage[b][#2][b]{#1}%
      {\fboxrule=0.2pt\fboxsep=0pt\fbox{%
        \includegraphics[width=20.22mm,height=25.47mm]{\jnllogo}}}%
  \endminipage}
  
\def\titleheaderfont{\fontsize{8pt}{8pt}\selectfont}
  
\def\stmtitleheader{%
  {\parskip=0pt%
   \parindent=0pt%
   \vspace*{\abovestmtitleheaderskip}%
   \minipage[t][][t]{\elstitleheaderwidth}%
  \par\vspace*{-12pt}%
   \elstitleheadboxa{\titleboxawidth}%
     {\titlegrayboxheight}{\titlegrayboxwidth}%
     \hspace*{\dimexpr(\titleblocksep-0.3pt)}%
   \elsjnllogoboxb{\elsjnllogowidth}{\elsjnllogoheight}%
   \par\vspace*{-3pt}%   
   \rule{\textwidth}{3pt}%   
  \vspace*{18pt}%
   \endminipage%
  }%
}  

\long\def\getSpaceLeft{%\global\@twocolumnfalse%
   \global\setbox0=\vbox{\hsize=\textwidth%
    \par\vspace*{12pt}%
    \MaketitleBox%
    \MakeabstractBox}%
   \global\setbox1=\vbox{\hsize=\textwidth
    \let\footnotetext\FNtext
    \printFirstPageNotes}%
    \xdef\noteheight{\the\ht1}%
    \xdef\titleheight{\the\ht0}%
    \@tempdima=\vsize
    \advance\@tempdima-\noteheight
    \advance\@tempdima-1\baselineskip
    \xdef\savefpageheight{\the\@tempdima}%    
    \setbox2=\vbox{\titlespancalculator{\titleheight}%
                  {\savefpageheight}{\textheight}{0}}%
}

%%Maketitle for medima
  \if@twocolumn
    \def\maketitle{%
      \iflongmktitle\getSpaceLeft
         \ifdim\noteheight>0pt%
			      \advance\@tempdima-1.35\baselineskip
         \fi%
         \setcounter{cnote}{0}%         
         \setcounter{tnote}{0}%
         \setcounter{fnote}{0}%
         \global\setbox\els@boxa=\vsplit0 to \@tempdima
         \box\els@boxa%
         \printFirstPageNotes%
         \par\resetTitleCounters
         \thispagestyle{pprintTitle}%
         \ifnum\savetitlepagespan>1\relax%
            \myfor{2}{\savetitlepagespan}{%
            \global\setbox\els@boxb=\vsplit0 to \textheight%\@tempdima              
            \twocolumn[\unvbox\els@boxb]}
         \else%
         \fi%       
         \twocolumn[\unvbox0]%
      \else
         \twocolumn[\vspace*{10pt}\finalMaketitle]\printFirstPageNotes
      \fi
     \gdef\thefootnote{\arabic{footnote}}%
     \ifpreprint%
        \global\advance\baselineskip by 6pt%
     \fi%
     }%
  \else
     \def\maketitle{%
        \iflongmktitle\getSpaceLeft
           \ifdim\noteheight>0pt%
			        \advance\@tempdima-1.35\baselineskip
           \fi%
           \setcounter{cnote}{0}%
           \setcounter{tnote}{0}%           
           \setcounter{fnote}{0}%           
           \global\setbox\els@boxa=\vsplit0 to \@tempdima
           \printFirstPageNotes%                      
           \unvbox\els@boxa%
           \par\resetTitleCounters
           \thispagestyle{pprintTitle}%
           \ifnum\savetitlepagespan>1\relax%
              \myfor{2}{\savetitlepagespan}{%
              \global\setbox\els@boxb=\vsplit0 to \textheight%\@tempdima              
              \unvbox\els@boxb}
           \else%
           \fi%              
           \unvbox0%
        \else
          \finalMaketitle\printFirstPageNotes
        \fi
        \gdef\thefootnote{\arabic{footnote}}%
        \ifpreprint%
           \global\advance\baselineskip by 6pt%
        \fi%
        }%
  \fi%


%% Title page header
\def\ps@MEDIMATitle{%
  \def\@oddhead{%
    %\stmtitleheader
   {\titleheaderfont%
   \hfil\@verso\ (\the\year)\hfil}%    
    }%
  \let\@evenhead\@empty
  \def\@oddfoot{%
      \ifpreprint%
        \ifnopreprintline\relax\else%
             Preprint submitted to \ifx\@journal\@empty%
               Elsevier%
           \else\@journal\fi\hfill\@date%
        \fi%
      \fi%
  }
  \let\@evenfoot\@oddfoot
}

\let\ps@pprintTitle\ps@MEDIMATitle

\def\ps@headings{%
   \def\@evenhead{{\titleheaderfont\rlap{\thepage}%
      \hfill\@verso\ (\the\year)\hfill\mbox{}}}
   \def\@oddhead{{\titleheaderfont\mbox{}%
      \hfill\@verso\ (\the\year)\hfill\llap{\thepage}}}
   \let\@oddfoot\relax
   \let\@evenfoot\@oddfoot
}

% Header for other than title page.
\pagestyle{headings}

% History info
\let\@received\@empty
\let\@finalform\@empty
\let\@accepted\@empty
\let\@availableonline\@empty
\let\@communicated\@empty
\def\received#1{\gdef\@received{#1}}
\def\finalform#1{\gdef\@finalform{#1}}
\def\accepted#1{\gdef\@accepted{#1}}
\def\availableonline#1{\gdef\@availableonline{#1}}
\def\communicated#1{\gdef\@communicated{#1}}

\def\receivedhead{Received}
\def\acceptedhead{Accepted}
\def\finalformhead{Received in final form}
\def\availableonlinehead{Available online}
\def\communicatedhead{Communicated by}

% Article info
\def\articleinfobox{%
    \parbox[t]{.25\textwidth}{%
    \vspace*{0pt}%
%    \hrule%        
%    \vspace*{6pt}%    
    \fontsize{8pt}{10pt}\selectfont%
    % \textit{Article history}:\\
    % \ifx\@received\@empty\relax
    % \else
    % \receivedhead~\@received\\
    % \fi
    % \ifx\@finalform\@empty\relax
    % \else
    % \finalformhead~\@finalform\\
    % \fi
    % \ifx\@accepted\@empty\relax
    % \else
    % \acceptedhead~\@accepted\\
    % \fi
    % \ifx\@availableonline\@empty\relax
    % \else
    % \availableonlinehead~\@availableonline
    % \fi
    % \ifx\@communicated\@empty\relax
    % \\[-2pt]
    % \else
    % \par
    % \vspace*{10pt}
    % \communicatedhead~\@communicated
    % \vspace*{12pt}
    % \fi
    % \hrule width 0.285\textwidth
    % \vspace*{1pc}
    \unhbox\keybox}
}

% Preprint Maketitle
\long\def\pprintMaketitle{\MaketitleBox}%



% Maketitle 
\long\def\MaketitleBox{%
  \resetTitleCounters
  \stmtitleheader%
  \def\baselinestretch{1}%
  \begin{\elsarticletitlealign}%
   \def\baselinestretch{1}%
%    \vspace*{7.5pc}
    \Large\@title\par\vskip18pt
    \normalsize
  \ifdoubleblind
%    \vspace*{2pc}
  \else
    \elsauthors\par\vskip10pt
    {\footnotesize\itshape\elsaddress}\par\vskip12pt
  \fi
\vspace*{-\baselineskip}%
  \end{\elsarticletitlealign}%
%  \vspace*{2pc}
%  \printFirstPageNotes%
}

\long\def\MakeabstractBox{%
\@tempdima=.335\textwidth%
\elsptputbox(-\strip@pt\@tempdima,0)(0,0)[tl]{\MakeartinfoBox}%
{%
\leftskip=\@tempdima%
\rule{.665\textwidth}{.2pt}\\[10pt]%\vskip10pt
    \noindent\begin{tabular*}{.665\textwidth}{@{}l@{}p{.665\textwidth}}
%     \hspace*{7pt}&A~B~S~T~R~A~C~T\\[8pt]
  \multicolumn{2}{@{}l@{}}{A~B~S~T~R~A~C~T}\\[8pt]
    \hline\\[-8pt]
    \end{tabular*}
    \par\noindent%
    \unvbox\absbox%
    \mbox{}\\[\belowabstractskip]%\rule{.665\textwidth}{.2pt}%\vskip10pt%    
    \noindent\hrule%
    \if@twocolumn%
      \vspace*{24pt}%
    \fi%    
}    
}

\long\def\MakeartinfoBox{%
\vtop{\hsize=.285\textwidth%
\noindent\rule{.285\textwidth}{.2pt}\\[10pt]%\vskip10pt%
 \noindent\begin{tabular*}{.285\textwidth}{@{}l@{}p{.285\textwidth}}
%   \hspace*{7pt}&A~R~T~I~C~L~E~~I~N~F~O\\[8pt]%
   \multicolumn{2}{@{}l@{}}{A~R~T~I~C~L~E\mbox{~~~}I~N~F~O}\\[8pt]
   \hline\\[-8pt]%
 \end{tabular*}%
 \par%
\noindent\articleinfobox\\[3pt]%\hrule
}
}

\long\def\finalMaketitle{%
  \resetTitleCounters
  \def\baselinestretch{1}%
   \MaketitleBox%
   \MakeabstractBox%
   \thispagestyle{MEDIMATitle}%
  \gdef\thefootnote{\arabic{footnote}}%
  }

 
\def\printFirstPageNotes{%
  \def\snm##1{##1}%
  \iflongmktitle
   \let\columnwidth=\textwidth\fi
  \ifdoubleblind
  \else
  \ifx\@tnotes\@empty\else\@tnotes\fi
  \ifx\@nonumnotes\@empty\else\@nonumnotes\fi
  \ifx\@cornotes\@empty\else\@cornotes\fi
  \ifx\@elseads\@empty\relax\else
   \let\thefootnote\relax
   \footnotetext{\ifnum\theead=1\relax
      \textit{e-mail:\space}\else
      \textit{e-mail:\space}\fi
     \@elseads}\fi
  \ifx\@elsuads\@empty\relax\else
   \let\thefootnote\relax
   \footnotetext{\textit{URL:\space}%
     \@elsuads}\fi
 \fi
  \ifx\@fnotes\@empty\else\@fnotes\fi
  \iflongmktitle\if@twocolumn
   \let\columnwidth=\Columnwidth\fi\fi
}

% Abstract
\renewenvironment{abstract}{%
  \global\setbox\absbox=\vtop\bgroup%
  \hsize=\textwidth%
  \leftskip=.335\textwidth%%
  \noindent\unskip\ignorespaces%
%  \hskip-1pt%
  }
%  {\mbox{}\newline%
%   \mbox{~}\hfill\copyright~\the\year\ %
%   Elsevier~B. V.~All~rights~reserved.\egroup%
%  }%



% Keyword
\def\keyword{%
  %\def\sep{\newline}%
  \def\sep{\unskip\ignorespaces,\space}%
  \def\MSC{\@ifnextchar[{\@MSC}{\@MSC[2000]}}%
%  \def\@MSC[##1]{\leavevmode\hbox {\it ##1~MSC:}\newline}%
  \def\@MSC[##1]{\leavevmode\hbox {\it ##1~MSC:}~}%
  \def\JEL{\newline\leavevmode\hbox {\it JEL:\space}}%
  \def\KWD{%
   \vspace*{10pt}\newline
%   \leavevmode\hbox {\it Keywords:}\newline}%
   {\it Keywords:}~}%
  \global\setbox\keybox=\hbox\bgroup\hsize=.3\textwidth%
  \fontsize{8pt}{10pt}\selectfont%
  \parskip\z@%
  \noindent%
  \ignorespaces}
\def\endkeyword{\egroup}

%% Other customization

% Enumerate
\def\labelenumii{\labelenumi.\arabic{enumii}}

% Caption
\def\figurename{Fig.}

\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip\footnotesize\bfseries
  \sbox\@tempboxa{#1.~#2}%
  \ifdim \wd\@tempboxa >\hsize
    #1.~#2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}

%\AtBeginDocument{\ifpreprint
%  \advance\baselineskip by 6pt
%\fi}

\def\TM{$^{\rm TM}$}

